Iterative Rational Krylov Algorithms for model reduction of a class of constrained structural dynamic system with Engineering applications

This paper discusses model order reduction of large sparse second-order index-3 differential algebraic equations (DAEs) by applying Iterative Rational Krylov Algorithm (IRKA). In general, such DAEs arise in constraint mechanics, multibody dynamics, mechatronics and many other branches of sciences and technologies. By deecting the algebraic equations the second-order index-3 system can be altered into an equivalent standard second-order system. This can be done by projecting the system onto the null space of the constraint matrix. However, creating the projector is computationally expensive and it yields huge bottleneck during the implementation. This paper shows how to find a reduce order model without projecting the system onto the null space of the constraint matrix explicitly. To show the efficiency of the theoretical works we apply them to several data of second-order index-3 models and experimental resultants are discussed in the paper.

==> csnameendcsname.tex <==
\relax 
\@setckpt{csnameendcsname\relax }{
\setcounter{page}{10}
\setcounter{equation}{16}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{1}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{5}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{1}
\setcounter{table}{1}
\setcounter{parentequation}{0}
\setcounter{caption@flags}{4}
\setcounter{continuedfloat}{0}
\setcounter{subfigure}{2}
\setcounter{subtable}{0}
\setcounter{ALC@unique}{0}
\setcounter{ALC@line}{0}
\setcounter{ALC@rem}{0}
\setcounter{ALC@depth}{0}
\setcounter{AlgoLine}{11}
\setcounter{algocfline}{3}
\setcounter{algocfproc}{3}
\setcounter{algocf}{3}
\setcounter{definition}{0}
\setcounter{conj}{0}
\setcounter{example}{3}
\setcounter{Maxaffil}{2}
\setcounter{authors}{4}
\setcounter{affil}{1}
}


==> preamble.tex <==
%\usepackage[hardware,software]{latexmacros/mymacros}
\usepackage{amsthm}
\usepackage{pgfplots}

\usepackage[vlined,longend,linesnumbered,ruled]{algorithm2e}
\providecommand{\dontprintsemicolon}{\DontPrintSemicolon}
\providecommand{\DontPrintSemicolon}{\dontprintsemicolon}
%\usepackage[colorlinks=true]{hyperref}

\usepackage[list=true]{caption,subcaption} %list=true enables listing
                                %of subfigures in the list of figures
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\pgfplotsset{every axis plot/.append style={line width=.75pt}}
%\DeclareMathOperator{\nul}{Null}
\DeclareMathOperator{\rang}{Rang}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Rank}{rank}
\DeclareMathOperator{\eps}{eps}
%\DeclareMathOperator{\Rel}{Re}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\det}{de}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newcommand\norm[1]{\left\lVert#1\right\rVert}

% some help for emacs tex user
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main" 
%%% TeX-PDF-mode:t
%%% auto-fill-function:nil
%%% mode:auto-fill
%%% flyspell-mode:nil
%%% mode:flyspell
%%% ispell-local-dictionary: "en_US"
%%% End: 
     


